Fast Consensus under Eventually Stabilizing Message Adversaries

This paper is devoted to deterministic consensus in synchronous dynamic networks with unidirectional links, which are under the control of an omniscient message adversary. Motivated by unpredictable node/system initialization times and long-lasting periods of massive transient faults, we consider message adversaries that guarantee periods of less erratic message loss only eventually: We present a tight bound of $2D+1$ for the termination time of consensus under a message adversary that eventually guarantees a single vertex-stable root component with dynamic network diameter $D$, as well as a simple algorithm that matches this bound. It effectively halves the termination time $4D+1$ achieved by an existing consensus algorithm, which also works under our message adversary. We also introduce a generalized, considerably stronger variant of our message adversary, and show that our new algorithm, unlike the existing one, still works correctly under it.

==> essentials.tex <==
\section{Motivation}

Much of the previous work on dynamic networks usually exhibits at least one
of the following characteristics:
\begin{compactitem}
  \item Connectedness in every round. Unnecessary, strong restriction.
  \item No eventual properties. Boot-up phases or transient faults require these, though.
  \item Undirected communication graphs. Not the general case, high price, inefficient.
\end{compactitem}

The contribution of this paper is to get rid of all these restrictions, i.e.,
we focus on directed communication graphs where no per-round connectivity
holds, but, eventually, the system stabilizes to some extent.

\section{General Definitions}

\begin{definition}[Root component]
A non-empty set of nodes $R \subseteq V$ is called a round $r$ root
component (or simply \emph{root} for brevity) if it holds that
$\forall p \in \Gr, q \in R : (p \ra q) \in \Gr \Rightarrow p \in R$.
We denote by $\roots(\Gr)$ the set of all root components of $\Gr$, resp.\
the single root of $\Gr$ and by $|R|$ the number of nodes that constitute
root component $R$.
\end{definition}

\begin{definition}[Shared root]
We say that a sequence $\SeqrI$ has a shared root $R$ if there
exists a root $R$ s.t.\ for all $r \in I : R \in \roots(\Gr)$.
\end{definition}

\begin{definition}[Maximal shared root]
Let $I=[a,b]$.
We call $R$ a maximal shared root of $\SeqrI$ if $R$ is a shared root
of $\SeqrI$ but neither of $(\G_r)_{r=a-1}^b$ nor $(\G_r)_{r=a}^{b+1}$. 
\end{definition}

\begin{definition}[Single-rooted sequence]
We call a sequence $\SeqrI$ single-rooted, or $R$-single-rooted,
if it has a unique shared root $R$ in $\SeqrI$, i.e.,
there exists a root component $R$ s.t.\
$\forall i, j \in I : \roots(\G_i) = \roots(\G_j) = R$.
\end{definition}

%Let $\G^u$ denote the underlying undirected graph of $\G$ and let the 
%diameter $d(\G^u)$ of a graph be defined as usual if $\G^u$ is connected, or the maximum
%diameter of its connected components if $\G^u$ is disconnected.
%
%\begin{definition}[Diameter $D$]
%We say that message adversary $A$ guarantees diameter $D$ if for all $\SeqInf \in A$,
%for all $\Gr \text{~of~} \SeqInf$ it holds that $D \geq d(\G^u_r)$.
%\end{definition}
%
%\begin{definition}[Hugo-reachability]
%Let $I=[a,b]$.
%$q$ is hugo-reachable from $p$ iff for every $\SeqrI$ with $|I| = hugo$,
%%if there is a path from $p$ to $q$ in $\Gr$ for all $r \in I$, then
%$cd^a(p,q) \leq hugo$.
%\end{definition}

Similarly to the classic ``happened-before'' relation,
%\cite{Lam78}
we say
that a process \emph{$p$ causally influences $q$ in round $r$}, denoted by
$(p \overset{r}{\leadsto} q)$, iff either (i) 
$q$ has an incoming edge
$(p \rightarrow q)$ from $p$ in $\G^r$, or (ii) if $q = p$, i.e., we assume that
$p$ always influences itself in a round. Given a sequence of communication graphs
$\G^r,\G^{r+1},\dots$, we say that there is an \emph{causal influence chain} 
of length $\ell \ge 1$ starting from $p$ in round $r$ to $q$, denoted by
$(p \overset{r[\ell]}{\leadsto} q)$, if there exists a
sequence of not necessarily distinct processes $p=p_0, \dots, p_\ell=q$ such that
$p_i\overset{r+i}{\leadsto}p_{i+1}$ for $0\le i < \ell$.
If $\ell$ is irrelevant, we just write $(p \overset{r}{\leadsto} q)$ or just $(p \leadsto q)$
and say that $p$ (in round $r$) causally influences $q$. 
This allows us to define the
notion of a dynamic causal distance between processes as given in \cref{def:dd}.

\begin{definition}[Dynamic causal distance]\label{def:dd}
Given a sequence of communication graphs $\G^r,\G^{r+1},\dots$,
the \emph{dynamic causal distance} $cd^r(p, q)$  from process $p$ (in round $r$) to process $q$ 
is the length of the shortest causal influence chain starting in $p$ in round $r$ and ending 
in $q$, formally $cd^r(p, q) := min\{\ell \colon (p \overset{r[\ell]}{\leadsto}q)\}$. We
define $cd^r(p, p) = 1$ and $cd^r(p,q) = \infty$ if $p$ never
influences $q$ after round $r$.
\end{definition}

\begin{lemma}[End to end delay]
\label{lem:information-propagation}
If there is a path from a process $p$ to $p'$ in every $G_r$ of a sequence
$\SeqrI$ with $I=[a,b]$ and $|I| = D$, then $cd^a(p,p') \leq D$.
\end{lemma}

\begin{proof}
Let $A(r)$ denote those processes whose round $a$ causal distance
from $p$ is at most $r-a+1$.
That is, $A(r) := \{ q \in \Pi | cd^a(p, q) \leq r - a + 1 \}$.
The complement of $A(r)$ is $A^C(r) := \Pi \setminus A(r)$.

We show the lemma by induction on $\ell$, $a \leq \ell \leq a+D-1$.
The induction hypothesis is that
$cd^a(p,p') \leq \ell - a + 1$ or $|A(\ell)| \geq \ell - a + 2$.
The latter implies the lemma since $A(b) = A(a+D-1) = \Pi$ because 
$A(b) \subseteq \Pi$.

Base, $\ell = a$: Since there is a path from $p$ to $p'$, $(p \ra q) \in G_a$ for
some $q \in \Pi$. Thus, $A(a) \supseteq \{ p, q \}$ and $|A(a)| \geq 2$.
If $q = p'$, we even have $cd^a(p, p') = 1$.

Step $\ell - 1$ to $\ell$: If the induction hypothesis implies
$cd^a(p, p') \leq \ell -1$, we are done.
Otherwise, since there is a path from $p$ to $p'$ in $\G_\ell$, it follows that
there are two processes $q, q'$, $q \in A(\ell -1), q' \in A^C(\ell -1)$ and
$(q \ra q') \in \G_\ell$.
Thus, $q' \in A(\ell)$ and $|A(\ell)| > |A(\ell-1)|$. By the induction hypothesis,
$|A(\ell)| \geq \ell - a + 2$.
\end{proof}

\Cref{lem:information-propagation} might tempt one to assume that a smaller
causal distance $cd^a(p,p')$ can be inferred if the maximal distance of $p'$
from $p$ for all $\Gr$ of $\SeqrI$ is somehow restricted.
This is not the case, however: Consider $\Gr$ to be a directed tree of height
three, where there is single root node $p$ and a single node $q$ in the second
level.
Each round let this node $q$ switch places with a new node $\neq p'$
from the third level.
In this scenario, $cd^a(p, p') = n-1$, even though the length of the path from
$p$ to $p'$ equals two in every round.

Given a network with a specified (spacial) distribution of the nodes that
allows less conservative guarantees of the end-to-end delay from
$p$ to $p'$ if a path from $p$ to $p'$ exists in all rounds, it makes
sense to introduce a system parameter to reflect this behavior.
We call this parameter $D$ and intuitively it is simply an upper bound
on the rounds it takes until a message is guaranteed to be forwarded from
a source to its destination if there exists a path from the source to the
destination for $D$ rounds.

It turns out that for solving consensus, it suffices to utilize this bound
only for the processes that are guaranteed to have an outgoing path to every
process in the system.
These are the members of the root $R$ in a $R$-single-rooted sequence $\SeqrI$ of
sufficient length $|I|$, as expressed in the following definition.

\begin{definition}[D]
$D$ is a bound s.t.\ if $\SeqrI$ is $R$-single-rooted and $|I| \geq D$, then
$\forall p \in R, \forall q \in \Pi, \forall x \in [a,b-D+1] : cd^x(p,q) \leq D$.
%all $q \in \Pi$ are $D$-reachable by any $p \in R$.
\end{definition}

%\begin{definition}[Dynamic causal diameter]
%We say that message adversary $A$ guarantees dynamic causal diameter $D$ if for all
%$\SeqInf \in A$, for all $\Gr \text{~of~} \SeqInf$ it holds that.
%If a subsequence $\SeqrI$ of length $|I| = |[a,b]| = D$ is $R$-single-rooted then
%$D \geq \max_{p \in R, q \in \Pi}(cd^x(p,q))$, for all $x \in [a, b-D+1]$.
%Let $\SeqrI$ be a $R$-single-rooted sequence.
%$D$ is the bound after which 
%\end{definition}

Note that $D < |V| = |\Pi|$ as an immediate consequence of
\cref{lem:information-propagation}.

\section{$n$-Based Message Adversary}

\subsection{Simple Version}

\begin{definition}[$\Safety$]
Let $\SeqrI$, with $I=[a,b]$, be any sequence with a maximal 
shared root $R$ and $|I| \geq n$.
We say a message adversary adheres to $\Safety$ if it guarantees that,
in every run,
at least $n$ subsequent rounds of $\SeqrI$ are single-rooted, i.e.,
there exists an interval $J \subseteq I$ with $|J| \geq n$ s.t.\
the sequence $(\Gr)_{r \in J}$ is single-rooted.
\end{definition}

\begin{definition}[$\Liveness$]
Let $I = [r_\text{stab}, b]$ and $|I| \geq 2n-2$.
A message adversary adheres to $\Liveness$ if it ensures that,
in every run,
there exists a
graph sequence $\SeqrI$ that has a shared root $R$ and there exists a round
$r_\text{sr}$, $r_\text{sr} \geq r_\text{stab} + n - 1$, s.t.\
$(\G_r)_{r=r_\text{sr}}^{r_\text{sr}+n-1}$ is $R$-single-rooted.
\end{definition}

\subsection{Advanced Version}

\begin{definition}[$\WeakSafety$]
Let $\SeqrI$, with $I=[a,b]$, be any sequence with a maximal 
shared root $R$ and $|I| \geq n$.
We say a message adversary adheres to $\WeakSafety$ if it guarantees that
at least one of the following holds for each $\SeqrI$ in every run:
\begin{compactitem}
\item At least $n$ consecutive rounds of $\SeqrI$ are single-rooted, i.e.,
      $\exists J \subseteq I : |J| \geq n \text{ and } (\G_r)_{r \in J}
      \text{ is } R\text{-single-rooted}$.
\item At least $n-|R^I|$ consecutive rounds of $\SeqrI$,
      starting at round $a+n+|R|-2$ or later, are single-rooted,
      i.e.,
      $\exists J=[a', b'] \subseteq I : |J| \geq n-|R^I|
      \text{ and } a' \geq a+ n+|R|-2
      \text{ and } (\G_r)_{r \in J} \text{ is } R\text{-single-rooted}$.
\end{compactitem}
\end{definition}

\begin{definition}[$\Liveness$]
Let $I = [r_\text{stab}, b]$.
We say a message adversary adheres to $\Liveness$ if it guarantees that
at least one of the following holds in every run:
\begin{compactitem}
\item There is a sequence $\SeqrI$ with $|I| = 2n-2$, a shared root $R$, and
      the last $n$ rounds of $\SeqrI$ are $R$-single-rooted, i.e.,
      $(\G_r)_{r=b-n+1}^b$ is $R$-single-rooted.
\item There is a sequence $\SeqrI$ with $|I| \geq 2n-1$ and a shared root $R$.
%      at least $n-|R^I|$ consecutive rounds of $\SeqrI$,
%      starting at round $\r_\text{stab}+n+|R|-2$ or later, are single-rooted.
%      Formally, 
%      $\exists J=[a', b'] \subseteq I : |J| \geq n-|R^I|
%      \text{ and } a' \geq a+ n+|R|-2
%      \text{ and } (\G_r)_{r \in J} \text{ is } R\text{-single-rooted}$.
\end{compactitem}
\end{definition}


\section{$D$-Based Message Adversary}

In order to define a message adversary that conforms to our desired system
behavior of eventual stability, we need two introduce two properties.

Firstly, we need the eventual stabilization itself,
a property that allows us to ensure liveness of
our solution algorithm, i.e., satisfy the termination criterion of consensus.
In a rather restricting (for the power of the adversary) form, this could
be a static network from some stabilization round onwards.
In \cref{def:liveness}, we
introduce a more relaxed and general variant that makes more
executions admissible and thus provides a significantly stronger adversary.
It requires only that every run has a single-rooted subsequence of a certain
finite length, i.e.,
there is only a single root component in every round of this subsequence and the
root members remain the same during the subsequence.
The interconnect may vary extensively during every round of the
subsequence, even the connections between the root members may change,
as long as the single-rootedness of the subsequence is preserved.
It is important that during this subsequence, it is
guaranteed that some process reaches the remainder
of the system.
If there is no such process, deciding correctly is impossible:
we can easily find executions where there are processes that have
disjoint sets of known input values throughout the entire run.
Perhaps surprisingly, it turns out that a length of the subsequence
that merely ensures that a process reaches everyone is still insufficient.
We show this in \cref{lem:adversary-tightness}.

Secondly, such a stabilization condition is not enough.
Consider for instance a run where all processes are disconnected until
eventually a chain forms, forever after, thereby satisfying the previous
stabilization condition.
In any correct solution algorithm the head of the chain, say $p$, must
eventually decide in some round $\tau$ on its initial value $x_p$.
However, then there is an execution, indistinguishable to $p$, where $p$
is disconnected until $\tau$, at which point it decides, but it is only
then that the chain forms with a head $q \neq p$ and $x_p \neq x_q$.

This is why we need a separate condition that allows our solution algorithm
to ensure the safety of consensus, i.e., agreement on the decided value.
The above example illustrates the main problem that we face here:
If we allow root components to stay stable for an arbitrary number of rounds,
then it is not possible for processes of the root component to tell whether
they are already in the subsequence in which it is guaranteed that they
reach everyone.

In previous work, this problem was usually solved by assuming that the
communication graph is connected and that it has a single root in every round.
Under eventual stabilization, however, this is not at all required.

\begin{definition}[$\Safety(X)$]
Fix any run $\SeqInf$. If there is a sequence $\SeqrI \subseteq \SeqInf$, s.t.\
$\SeqrI$ has a maximal shared root $R$ and $|I| \geq X$, then there is a $R$-single-rooted
sequence $(\G_r)_{r \in J} \subseteq \SeqrI$ with $|J| \geq X$.
\end{definition}

\begin{definition}[$\Liveness(X)$] \label{def:liveness}
A message adversary adheres to $\Liveness(X)$ if it ensures that,
in every run $\SeqInf$,
there exists a
sequence $\SeqrI \subseteq \SeqInf$
with $I = [\aGST, \bGST]$
s.t.\ all of the following hold:
\begin{compactitem}
\item $|I| \geq X$
\item $\SeqrI$ has a shared root $R$.
\item There is a round
$\rSR > \aGST+D$, s.t.\
$(\G_r)_{r=\rSR}^{\rSR+D-1}$ is $R$-single-rooted.
\end{compactitem}
\end{definition}

\section{Impossibility Proofs}

\begin{theorem}\label{thm:adversary-tightness}
Solving consensus is impossible under adversary
$\langle \Safety(X-D+1)$, $\Liveness(X) \rangle$
for any $X \leq 2D$.
\end{theorem}

\begin{proof}
Assume an algorithm $A$ exists that solves consensus under this adversary.
In particular, $A$ solves consensus in the following execution
$\varepsilon$:
Let all processes start with input value $0$.
First, the nodes form a chain of length $D$ with a single head but two
tails $p$ and $q$ from round $1$ to round $X$.
From round $X+1$ on, the nodes form a chain with alternating heads $p$ and
$q$:
The processes form a chain, every even round there is an edge from $p$ to
$q$, while every odd round there
is an edge from $q$ to $p$ and there are no other incoming edges to either $p$
or $q$.
It is not hard to see that this execution is in accordance with the
guarantees of the adversary.
Thus, by validity and termination, processes $p$ and $q$ must eventually have
decided $0$ in some round $\tau$.

We now present an admissible execution $\varepsilon'$ for $A$ that is
indistinguishable for $p$ and $q$ until round $\tau$ but some processes
will eventually decide $1$, which provides a contradiction to the assumption
that a correct $A$ exists.

Let $\Pi_{\varepsilon}$ denote the set of processes that were part
of execution $\varepsilon$
and let $\Pi_{\varepsilon'} = \Pi_{\varepsilon} \cup \{ p', q'\}$.
Let all processes of $\Pi_\varepsilon$ start with input $0$ and let $p'$ and
$q'$ start with $1$.
Until round $\tau$ let there be an edge from $p'$ to $q'$ in every even round
and an edge from $q'$ to $p'$ in every odd round and let there be no other 
outgoing edges from $p'$ or $q'$.
For the first $X-D$ rounds let the nodes of $\Pi_\varepsilon$ behave the
same as in $\varepsilon$.
In round $X-D+1$ let there be an edge from $p$ to the head of the chain.
From round $X-D+2$ until round $\tau$, let the nodes $\Pi_\varepsilon$
again behave as in $\varepsilon$.
From round $\tau$ on, let the graph be a directed star, going out from $p'$
to every node in the system.
By validity, $p'$ will thus eventually decide $1$, as asserted.
\end{proof}

\section{Algorithm}

\newcommand\lock[1]{\mathtt{lock}_{#1}}
\newcommand\round{\mathtt{r}}
\newcommand\lockround{\mathtt{lockRound}}
\newcommand\counter{\mathtt{count}}
\newcommand\lockval{\ell}
\newcommand\Root{R}

\begin{figure*}[ht!]
 \centering
 \begin{tikzpicture}[
   cond/.style={draw, rounded corners, align=left},
   branch/.style={draw, align=left},
   link/.style={->,>=stealth'}]
   \def\yorigin{-1}
   \def\dx{8}
   \def\dy{-2}
   \newcommand\yes[2]{\draw[link] (#1) -- node[auto] {yes} (#2)}
   \newcommand\no[2]{\draw[link] (#1) -- node[auto, near start] {no} (#2)}
   \newcommand\notip[2]{\draw[] (#1) -- node[auto, near start] {no} (#2)}

%   \node[branch] (initialization) at (0, \yorigin+2)
%      {\textbf{Initialization:} \\
%      $\lock{p} := x_p$};

   \node[draw, densely dotted] (start) at (0,\yorigin) {start of round $r$ computation}; 
   \node[draw, densely dotted] (end) at (\dx,\yorigin) {end of round $r$ computation}; 
   \node[cond] (c1) at (0,\dy)
      {\textbf{c1:}\\ Is there a single root $R$ in $\ApproxGp{r-D}$?}; 
   \node[branch] (b1) at (0,2*\dy)
      {\textbf{b1:}\\ Set $\lock{p}$ to maximum $\lock{q}$ value \\ of any process $q \in R$};
   \node[cond] (c2) at (0, 3*\dy)
      {\textbf{c2:}\\ Is $R$ a shared root of some $(\ApproxGp{r})_{r \in I}$ \\ with
      $I=[a,b], |I| > D$ and $r-D \in I$?};
   \node[cond] (c3) at (0, 4*\dy)
      {\textbf{c3:}\\ Is $|R| = 1$?};
   \node[branch] (b3) at (2/3*\dx,4*\dy)
      {\textbf{b3:}\\ decide  $y_p := \lock{p}$};
   \node[cond] (c4) at (0,5*\dy)
      {\textbf{c4:}\\ Is $R$ a root of $\ApproxGp{a-1}$ or $\ApproxGp{b+1}$?};
   \node[branch] (b4) at (0,6*\dy)
      {\textbf{b4:}\\ decide  $y_p := \lock{p}$};

   \def\Xa{\dx, \dy}
   \def\Xb{\dx, 3*\dy}
   \def\Xc{\dx, 4*\dy}
   \def\Xd{\dx, 5*\dy}
   \def\Xe{\dx, 6*\dy}
   
   \draw[link] (start) -- (c1);
   \draw[link] (b1) -- (c2);
   \yes{c1}{b1};
   \notip{c1}{\Xa};
   \yes{c2}{c3};
   \notip{c2}{\Xb};
   \no{c3}{b3};
   \draw (b3) -- (\Xc);
   \yes{c3}{c4};
   \notip{c4}{\Xd};
   \yes{c4}{b4};
   \draw (b4) -- (\Xe);
   \draw[link] (\Xe) -- (end);

 \end{tikzpicture}

 \caption{Algorithm for round $r$ and process $p$. Let $\ApproxGp{r}$ denote
   $p$'s view of $\G_r$ and let $\lock{p} = x_p$ initially.} \label{fig:algorithm}
\end{figure*}

\section{Graph Approximation}

At the core of our algorithm lies the simple mechanism
that each process sends out its current local view of the communication graph
sequence and $\ell$.
We assume that processes update their own view of the communication graph
sequence with the views they received from other nodes of the graph.
This full-information approach incurs sending and storing a large amount
of redundant information and is done to focus the exposition of the
algorithm on the essential concepts.
We provide hints for a more efficient approach in
\cref{sec:memory-message-complexity}.

We don't want to go into the details of how to implement such an approximation
here.
A fitting algorithm, along with a correctness proof, can be found in
\cite{BRS12:sirocco}.
As in that algorithm, we assume here that processes under-approximate the
actual communication graph, i.e., they do not fabricate edges in their
approximation.
In particular, if a process $p$ receives a round $r$ message from $q$ but
$p$ has not yet learned whether $q$ had an in-edge in round $r$, $p$ will
assume (until it learns more) that $q$ had no such in-edge.

We conclude this section by making some statements about the basic
learning behavior, nodes can achieve in a full-information protocol.
\todo{Some informal introduction to the lemmas.}

\begin{lemma} \label{lem:root-detection}
Let $\SeqrI$ be any communication graph sequence with shared
root $R$ and $|I| \geq D+2$, $I = [a, b]$.
Then, a process $p$ that received a message from every $q \in R$, sent in round
$a+D+1$, detects that $R$ was shared root of $\Seqr{a}{a+D}$.
If, in addition, $|R|=1$, then $p$ even detects that $R$ was shared root
of $\Seqr{a}{a+D+1}$.
\end{lemma}

\begin{proof}
For $|R| \geq 1$, we have that an arbitrary process $p$ received a message from
every $q \in R$ by our assumption.
Since we are dealing with a full-information protocol, $p$ received the round
$a+D$ graph approximation of every $q \in R$, which contains the round $a+D$
in-edges of $q$.
Thus, $p$ learned all in-edges, any $q \in R$ had in $(\Gr)_{r=1}^{a+D}$.
Consequently, $p$ can calculate the root component of this subsequence.

For $|R| = 1$, let us distinguish two cases:
If $p$ received a message from $R = \{ q \}$, sent in round $a+D+2$ or later,
$p$ learned $q$'s round $a+D+1$ graph approximation.
Hence, $p$ also learned that $q$ had no in-edges
since $\Seqr{a+D+1}{a+D+1}$ is actually $\{ q \}$-single-rooted.
If $p$ did not receive this message, it nevertheless received one
sent in round $a+D+1$ by the assumptions of the lemma.
Process $p$ hence learns that $q$ had an out-edge in round $a+D+1$ and assumes,
the way we sketched the graph approximation, that $q$ had no in-edge
in round $a+D+1$.
Thus, in both cases, $p$ detects that $\Seqr{a}{a+D+1}$ was $R$-single-rooted.
\end{proof}

\begin{lemma} \label{lem:root-propagation}
Let $\SeqrI$ be any $R$-single rooted sequence of communication graphs with
$|I| \geq D+1$, $I=[a,b]$.
Then, every process $p$ detects in round $a+D$
that $\Seqr{a}{a}$ was $R$-single-rooted.
\end{lemma}

\begin{proof}
It follows from \cref{lem:information-propagation} that, at latest in round
$a+D$, $p$ received a message sent by every $q \in R$ in round $a+1$.
Since we are dealing with a full-information protocol,
$p$ hence learns in round $a+D$ the graph approximation of every $q \in R$
from round $a$.
This implies that $p$ learns the in-edges of every $q \in R$.
Since we assume that $\SeqrI$ is $R$-single rooted and our graph approximation
is an under-approximation,
$p$ can thus easily determine the root component of $\Seqr{a}{a}$.
\end{proof}

\section{Correctness Proof}

We now show the following \cref{thm:correctness} by establishing that the
algorithm from \cref{fig:algorithm} asserts the three correctness
conditions of consensus.

\begin{theorem} \label{thm:correctness}
The algorithm from \cref{fig:algorithm} solves consensus.
\end{theorem}

\begin{lemma}
The algorithm ensures validity.
\end{lemma}
\begin{proof}
Observe that decisions occur only in b3 and b4 and on a value of $\lock{p}$.
Validity is implied since $\lock{p} = x_p$ initially for all $p \in \Pi$.
\end{proof}

\begin{lemma}
The algorithm ensures agreement.
\end{lemma}
\begin{proof}
Let $\lock{p}(r)$ denote the value of $\lock{p}$ at process $p$ in round $r$.
Observe that decisions occur only in b3 and b4 and a value of $\lock{p}$.
To show agreement, it thus suffices to show the following:
Let $r$ be the round when it happens for the first time in a run that
some process $p$ assigns $v$ to $y_p$.
Then,
all $\lock{q}$ values are the same and never change anymore, or, more
precisely,
for all $q \in \Pi$, for all $r' \geq r$ it holds that $\lock{q}(r') = v$.

Assume that process $p$
indeed assigned $y_p := v$ in round $r$ and this was the first time a process
did so in the current run.
By the code of the algorithm, $c2$ to $c4$,
$p$ must have observed a $R$-single rooted
$\SeqrI$ with $I=[a,b], r-D \in I$ and
either $|I| > D+1$ or $|R|>1$ and $|I| > D$.
Accordingly, let $x = D+2$ if $|R| = 1$ and $x=D+1$ if $|R| > 1$.
Also, note that the maximum $\lock{q}$ value of any $q \in R$ must have
been $v$.

Note that for $\SeqrI$, \cref{lem:root-propagation} is applicable
since $\Safety(D+1)$ ensures us the existence of a $R$-single-rooted
subsequence $(\G_r)_{r \in I'}$ with $I' \subseteq I$ and $|I'| \geq D+1$.

\Cref{lem:root-propagation} implies that by round $a+x$ all processes
$q \in \Pi$ have observed that $G_a$ was $R$-single-rooted.
But then, they passed $c1$ and set $\lock{q} := v$ in round $a+x$.

Any process $q'$ that becomes member of a root in any round $r' \geq a+x$
thus has already $\lock{q'} = v$ and hence, for all $q \in \Pi$,
any value
assigned to $\lock{q}(r')$ in b1 is equal to $v$.
Since $r \geq a+x$, this proves the Lemma.
\end{proof}

\begin{lemma}
The algorithm terminates at latest in round $\rSR+D-1$.
\end{lemma}
\begin{proof}
Since our message adversary satisfies $\Liveness(2D+1)$,
$R$ is a shared root of $\SeqrI$ with $I=[\aGST, \bGST]$ and
$|I| \geq 2D+1$.

By \cref{lem:information-propagation},
in a full-information protocol,
every $p \in \Pi$
receives, no later than in round $\rSR+D-1$, a message sent from
every $q \in R$ in round $\rSR-1$.
Since $\rSR > \aGST + D$, $p$ in fact received a message from $q$
for all $D+2$ rounds of $[\aGST, \aGST+D+1]$.
Let us distinguish two cases.

If $|R| > 1$,
\cref{lem:root-detection} implies that $p$ detects that
$(\Gr)_{r=\aGST}^{\aGST+D}$ was $R$-single-rooted.
By the code of the algorithm,
$p$ thus decides via b3 at latest in round $\rSR+D-1$.

If, on the other hand, $|R| = 1$,
\cref{lem:root-detection} implies that $p$ detects that
$(\Gr)_{r=\aGST}^{\aGST+D+1}$ was $R$-single-rooted.
Therefore, $p$ will decide via b4 at latest in round $\rSR+D-1$.
\end{proof}


==> majinf-estable.tex <==
 
\begin{comment}
\begin{lemma}
$\EStable(D) \subseteq \mathtt{VSRC}(n, 3D + H) + \mathtt{MAJINF}(1)$
\end{lemma}

\begin{proof}
  First let us rephrase the adversary $\mathtt{VSRC}(n, 3D + H) + \mathtt{MAJINF}(1)$.
  \begin{compactitem}
  \item For any sequence $\sigma$ of $\mathtt{VSRC}(n, 3D+H)$, there exist a round $\rGST$ and
    a set of root components $\mathcal{R}$ such that $\mathcal{R} = \roots(\Gr)$
    with $|\mathcal{R}| \leq n$
    for all $\Gr$ of $\Seqr{\rGST}{\rGST+3D+H-1} \subseteq \sigma$.
  \item Let For any sequence $\sigma$ of $\mathtt{MAJINF}(1)$ it holds that 
  \end{compactitem}
\end{proof}
\end{comment}

